A Stackelberg Game Approach to Control the Overall Load Consumption of a Residential Neighborhood

This paper formulates a Stackelberg game between a coordination agent and participating homes to control the overall load consumption of a residential neighborhood. Each home optimizes a comfort-cost trade off to determine a load schedule of its available appliances in response to a price vector set by the coordination agent. The goal of the coordination agent is to find a price vector that will keep the overall load consumption of the neighborhood around some target value. After transforming the bilevel optimization problem into a single level optimization problem by using Karush-Kuhn-Tucker (KKT) conditions, we model how each home reacts to any change in the price vector by using the implicit function theorem. By using this information, we develop a distributed optimization framework based on gradient descent to attain a better price vector. We verify the load shaping capacity and the computational performance of the proposed optimization framework in a simulated environment establishing significant benefits over solving the centralized problem using commercial solvers.

==> conclusions.tex <==
\section{Conclusions}

TO COME ...

==> optimization.tex <==
\section{PROPOSED OPTIMIZATION PROBLEM}
%
%Consider a power grid managed by a coordination agent serves $N$ participating homes equipped with $M$ appliances introduced previously, it is possible to design a Stackelberg game to control the total load consumption of the community.
Consider a power grid managed by a coordination agent serves $N$ participating homes equipped with $M$ appliances introduced previously. The total load consumption of the community can be controlled by formulating a Stackelberg game where the coordination agent is the leader and the homes are followers. In this game, the coordination agent announces a price vector, then homes automatically adjust the power consumption schedule of the available appliances by considering their individual preferences to minimize their cost functions.
%
Suppose that ${p_{ij}}(t)$ is a decision variable denoting the load consumption of home $i$ for appliance $j$ at time point $t$,\cmmnt{consumed by appliance $j$ in home $i$ at time point $t$.} and \[\boldsymbol{p}_i=\left[p_{i1}(0)\ ...\ p_{i1}(K-1)\ ... \ p_{iM}(0)\ ...\ p_{iM}(K-1)\right]^T\] is a vector of decision variables denoting the load schedule of the home $i$ over the next $K$ time intervals. Each home defines a set of comfort related linear constraints according to its preferences, and these constraints form the polyhedron $\P_i = \{\boldsymbol{p}_i\ |\ G_i\boldsymbol{p}_i\leq h_i\},\ \forall i$. Hence, the comfort of home $i$ can be ensured as long as $\boldsymbol{p}_i \in \Pi$. Although determining $\boldsymbol{p}_i$ by solving an optimization problem, which minimizes the electricity bill according to the announced price vector, $\boldsymbol{\pi}$, over the set $\P_i$, is promising, there is an oversight in this strategy.\cmmnt{this can be insufficient to reflect the user behaviour.} Each home has different consumption habits, thus a desirable load schedule for each appliance. As any deviation from this schedule causes a social discomfort in the users, the amount of the deviations must be taken into account as well as the electricity bill while determining the load schedule of homes. Then, for a given price vector $\boldsymbol{\pi}$, the optimization problem solved by home $i$  is as follows:
% \begin{equation}
% \begin{split}
% &\boldsymbol{p}_i^*:=f_i(\boldsymbol{p}_i, \boldsymbol{\pi})=\\[0.75em]
% &\argmin_{\boldsymbol{p}_i\in \P_i} \sum_{j=1}^M\sum_{t=0}^{K-1} p_{ij}(t)\pi(t)+\sum_{j=1}^M\sum_{t=0}^{K-1}c_{ij}\left(p_{ij}(t)-\overline{p_{ij}}(t)\right)^2,\label{opt_eq_1} 
% \end{split}
% \end{equation}
\begin{equation}
\begin{split}
\boldsymbol{p}_i^*:=f_i(\boldsymbol{p}_i, \boldsymbol{\pi})&=\argmin_{\boldsymbol{p}_i\in \P_i} \sum_{j=1}^M\sum_{t=0}^{K-1} p_{ij}(t)\pi(t)\\
&+\sum_{j=1}^M\sum_{t=0}^{K-1}c_{ij}\left(p_{ij}(t)-\overline{p_{ij}}(t)\right)^2,\label{opt_eq_1} 
\end{split}
\end{equation}
where $c_{ij}$ represents the importance of appliance $j$ for home $i$, and $\overline{p_{ij}}(t)$ represents the desirable load of appliance $j$ in home $i$ at time point $t$. While the first term in Equation \eqref{opt_eq_1} minimizes the electricity bill, the second term penalizes the deviations from the desirable load curve.

On the other hand, the coordination agent wants to keep the total load consumption of the community under control while minimizing the total social discomfort of the community by choosing an appropriate electricity price vector $\boldsymbol{\pi}$. Therefore, for a given $\boldsymbol{\pi}$, $\boldsymbol{p}^*$ denotes the optimal load consumption vector of the neighborhood, e.g., $\boldsymbol{p}^*=\left[(\boldsymbol{p}_1^*)^T\ ...\ (\boldsymbol{p}_N^*)^T\right]^T$, and the objective function of the coordination agent can be expressed as follows:
\begin{flalign}
\notag f(\boldsymbol{p}^*, \boldsymbol{\pi}) :=&\sum_{t=0}^{K-1}\left(Q(t) - \sum_{i=1}^N\sum_{j=1}^M p_{ij}^*(t)\right)^2\\
&+\sum_{i=1}^N\sum_{j=1}^M\sum_{t=0}^{K-1}c_{ij}\left(p_{ij}^*(t)-\overline{p_{ij}}(t)\right)^2,\label{opt_eq_2}
\end{flalign}
where $Q(t)$ represents the targeted aggregate power consumption level at time $t$. While the first term in Equation \eqref{opt_eq_2} minimizes the deviation from $Q(t)$ at any time interval $t$, the second term minimizes the total social discomfort of the neighborhood. Therefore, the coordination agent seeks a price vector minimizing her objective function. However, as the coordination agent has to act in accordance with some regulations, the electricity price cannot exceed a certain threshold. Similarly, the coordination agent cannot lower the price freely because of the cost of generating electricity. We assume that these requirements are satisfied as long as $\boldsymbol{\pi} \in \Pi$. The resulting bilevel optimization problem considered in this paper is as follows:
\begin{align}
\min_{\pi \in \Pi}\quad &f(\boldsymbol{p}^*, \boldsymbol{\pi})\label{opt_eq_3}\\
\text{s.t.} \quad & \boldsymbol{p}_i^*:=f_i(\boldsymbol{p}_i, \boldsymbol{\pi}), \quad \forall i.\label{opt_eq_5}
%\quad & \boldsymbol{\pi} \in \Pi.
\end{align}


For a given price, the home level optimization problem is a convex quadratic program. Therefore, the bilevel problem given in Equations \eqref{opt_eq_3}-\eqref{opt_eq_5} can be reformulated as a single level problem by replacing the optimality constraint given in Equation \eqref{opt_eq_5} with the KKT conditions of each home:
\begin{align}
\min_{\substack{\boldsymbol{p}_1, \dots, \boldsymbol{p}_N,\\ \boldsymbol{\lambda}_1, \dots, \boldsymbol{\lambda}_N, \\\boldsymbol{\pi} \in \Pi}}\quad &f(\boldsymbol{p}, \boldsymbol{\pi})\label{opt_eq_6}\\[0.5em]
\text{s.t.} \qquad  &\nabla_{\boldsymbol{p}_i}f_i(\boldsymbol{p}_i, \bpi) + G_i^T\boldsymbol{\lambda}_i = 0, \qquad \forall i,\label{opt_eq_7}\\
\qquad & \text{Diag}(\boldsymbol{\lambda}_i)\left(G_i\boldsymbol{p}_i-h_i\right) =0,\qquad \forall i,\label{opt_eq_8}\\
\qquad & G_i\boldsymbol{p}_i \leq h_i,\qquad\qquad\qquad\qquad\ \forall i,\label{opt_eq_9}\\ 
\qquad & \boldsymbol{\lambda}_i \geq 0,\qquad\qquad\qquad\qquad\qquad \forall i,\label{opt_eq_10}
\end{align}
where $\boldsymbol{\lambda}_i$ is a vector of the dual variables corresponding to the constraints in the set $\P_i$. Since the objective function of each home is quadratic, the stationarity constraints given in Equation \eqref{opt_eq_7} are linear. However, the constraints enforcing the complementary slackness condition are non-convex. Thus, the optimization problem in Equations \eqref{opt_eq_6}-\eqref{opt_eq_10} is a non-convex {\em{Quadratically Constrained Quadratic Program}} (QCQP).  \cmmnt{which make the optimization problem given in Equations \eqref{opt_eq_6}-\eqref{opt_eq_10} hard to solve.}


